Semi-Weakly Supervised Object Kinematic Motion Prediction

Given a 3D object, kinematic motion prediction aims to identify the mobile parts as well as the corresponding motion parameters. Due to the large variations in both topological structure and geometric details of 3D objects, this remains a challenging task and the lack of large scale labeled data also constrain the performance of deep learning based approaches. In this paper, we tackle the task of object kinematic motion prediction problem in a semi-weakly supervised manner. Our key observations are two-fold. First, although 3D dataset with fully annotated motion labels is limited, there are existing datasets and methods for object part semantic segmentation at large scale. Second, semantic part segmentation and mobile part segmentation is not always consistent but it is possible to detect the mobile parts from the underlying 3D structure. Towards this end, we propose a graph neural network to learn the map between hierarchical part-level segmentation and mobile parts parameters, which are further refined based on geometric alignment. This network can be first trained on PartNet-Mobility dataset with fully labeled mobility information and then applied on PartNet dataset with fine-grained and hierarchical part-level segmentation. The network predictions yield a large scale of 3D objects with pseudo labeled mobility information and can further be used for weakly-supervised learning with pre-existing segmentation. Our experiments show there are significant performance boosts with the augmented data for previous method designed for kinematic motion prediction on 3D partial scans.

==> figures/axis_dgcnn.tex <==
\begin{figure*}[!t]
    \centering
    % \includegraphics[width=\linewidth]{latex/images/axis_selection_network.png}
    \includegraphics[width=\linewidth]{latex/images/axis_dgcnn.pdf}
    
\caption{DGCNN encoder used in axis selection network} 
\label{fig:axis_dgcnn}
\end{figure*}


==> figures/axis_fc.tex <==
\begin{figure}[h]
    \centering
    % \includegraphics[width=\linewidth]{latex/images/axis_selection_network.png}
    \includegraphics[width=\linewidth]{latex/images/axis_fc.pdf}
    
\caption{Fully connected layer used in axis selection network} 
\label{fig:axis_fc}
\end{figure}


==> figures/axis_selection_network.tex <==
\begin{figure}[!t]
    \centering
    % \includegraphics[width=\linewidth]{latex/images/axis_selection_network.png}
    \includegraphics[width=\linewidth]{latex/images/axis_selection_network (optimized).pdf}
    
\caption{The input to the network includes the original point clouds and the transformed point clouds after applying the candidate motion, associated with point-wise one-hot label indicating whether the point belongs to the mobile or reference part. The output is a feasibility score for the relative motion.} 
\label{fig:axis_net}
\end{figure}


==> figures/fig_axis_example.tex <==
\begin{figure}[]
    \centering
    % \includegraphics[width=\linewidth]{latex/images/axis_select_example.png}
    \includegraphics[width=0.96\linewidth]{latex/images/axis_select_example (optimized).pdf}
\caption{Example of positive and negative transformed point clouds for training axis selection network.}
\label{fig:axis_select_example}
\end{figure}


==> figures/fig_result_mobility.tex <==
\begin{figure*}%[!t]
    \centering
    \includegraphics[width=\linewidth]{latex/images/more_mobility (optimized).pdf}
\caption{ Visual comparison of results obtained by \emph{GNN\_coarse}, \emph{GNN\_fine}, \emph{OBB\_coarse} and \emph{OBB\_fine} on pre-segmented point clouds. \emph{OBB\_fine} always predict high quality motion parameters compare to other method owing to the fine characterization of the motion type and the use of OBB priors and introduction of the interaction region.}
\label{fig:result_mobility}
\end{figure*}


==> figures/fig_result_partnet.tex <==
\begin{figure*}%[!t]
    \centering
    \includegraphics[width=0.95\linewidth]{latex/images/result_partnet2 (optimized).pdf}

\caption{ Pseudo labels predicted by our method on PartNet. The first and third column are the input point clouds with fine-grained segmentation, and the second and last column are the merge segmentation and motion parameters predicted by our method}
\label{fig:result_partnet}
\end{figure*}


==> figures/obb_candidate.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.3\textwidth]{latex/images/obb_candidate.png}
\caption{OBB candidate.}
\label{fig:obb_candidate}
\end{figure}


==> figures/tab_amountlist.tex <==
\begin{table}[h]
% \scriptsize\addtolength{\tabcolsep}{-2pt}
\addtolength{\tabcolsep}{-3pt}
\centering
%\begin{center}
\begin{tabular}{c|c}\toprule
joint            &  motion amounts  \\ \midrule 
\emph{P}               &  -0.38, -0.27, -0.16, 0.16, 0.27, 0.38 \\
\emph{R}               &  -80°, -60°, -45°, -30°, 30°, 45°, 60°, 80° \\
\emph{PR}   &  (-0.02, 60°), (-0.02, 60°), (0.02, 90°), (0.02, 90°) \\ \bottomrule 
\end{tabular}
\caption{Motion amount list for different types of joints. \emph{P}, \emph{R} and \emph{PR} represent the prismatic, revolute and both joints.}
\label{tab:amount_list}
\end{table}


==> figures/tab_dsg.tex <==
% \begin{table*}[t]
% \footnotesize
% \addtolength{\tabcolsep}{-2pt}
% \centering
% %\begin{center}
% \begin{tabular}{c|c|ccc|c|cc} \toprule 
% \multirow{2}{*}{Category}           & \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Part-based Metrics}                                           & Joint States       & \multicolumn{2}{c}{Joint Parameters}      \\ 
%                                     &                         & Rotation Error °↓         & Translation Error↓         & 3D IoU ↑                & Error↓             & Angle Error°↓      & Distance Error↓      \\ \midrule 
% \multirow{2}{*}{StorageFurniture}     & ANCSH   & 40.01 47.41 43.77  & 0.400 0.400 0.379	 &	62.5 20.7 17.4 &	30.91 27.11 	& 9.22 6.39 &	0.063 0.061  \\
%                           & ANCSH (Dsg-net) & \textbf{40.00 45.53 42.01} & \textbf{0.349 0.373 0.308} & \textbf{66.6 23.0 21.4} & \textbf{30.80 25.77} & \textbf{1.54 1.53}  &  \textbf{0.061 0.056}   \\ \bottomrule 
% \end{tabular}
% \caption{Quantitative results of ANCSH for motion prediction on partial point clouds with and without using shapes from DSG-Net for data augmentation.}
% \label{tab:result_dsg}
% \end{table*}

% \begin{table}[t]
% \footnotesize
% \addtolength{\tabcolsep}{-2pt}
% \centering
% %\begin{center}
% \begin{tabular}{c|ccc|c|cc} \toprule 
% \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Part-based Metrics}  & Joint States       & \multicolumn{2}{c}{Joint Parameters}      \\ 
%   & Rota. Err.         & Trans. Err.         & 3D IoU                & Err.             & Ang. Err      & Dis. Err.      \\ \midrule 
%     ANCSH   & \thead{40.0 \\ 47.4 43.7}    & \thead{ 0.40 \\ 0.40 0.37}  	 &	\thead{ 62.5 \\ 20.7 17.4}   & 	\thead{30.9 \\ 27.1} 	& \thead{9.2 \\ 6.3} &	\thead{0.063 \\ 0.061}  \\
%     ANCSH(Dsg) & \thead{ \textbf{40.0  } \\ \textbf{45.5 42.0} } &    \thead{ \textbf{0.34 } \\ \textbf{0.37 0.30} }  &  \thead{ \textbf{66.6} \\ \textbf{23.0 21.4} }  & \textbf{\thead{30.8 \\ 25.7}} & \textbf{\thead{1.5 \\ 1.5}}  &  \textbf{\thead{0.061 \\ 0.056}}   \\ \bottomrule 

% \end{tabular}
% \caption{Result on partial scans using generated shapes from Dsg-net as augmented data.}
% \label{tab:result_dsg}
% \end{table}


%%%%%%% rebuttal
\begin{table}[t]
\footnotesize
\addtolength{\tabcolsep}{-4pt}
\centering
%\begin{center}
\begin{tabular}{c|ccc|c|cc} \toprule 
 Method & Rota. Err.   & Trans. Err.   & 3D IoU     & Joint Err.  & Ang. Err   & Dis. Err.      \\ \midrule 
    ANCSH   & \thead{40.0 \\ 47.4 43.7}    & \thead{ 0.40 \\ 0.40 0.37}  	 &	\thead{ 62.5 \\ 20.7 17.4}   & 	\thead{30.9 \\ 27.1} 	& \thead{9.2 \\ 6.3} &	\thead{0.063 \\ 0.061}  \\
    \thead{ANCSH\\(DSG) }& \thead{ \textbf{40.0  } \\ \textbf{45.5 42.0} } &    \thead{ \textbf{0.34 } \\ \textbf{0.37 0.30} }  &  \thead{ \textbf{66.6} \\ \textbf{23.0 21.4} }  & \textbf{\thead{30.8 \\ 25.7}} & \textbf{\thead{1.5 \\ 1.5}}  &  \textbf{\thead{0.061 \\ 0.056}}   \\ \bottomrule 

\end{tabular}
\vspace{-1mm}
\caption{
Quantitative results of ANCSH for motion prediction on partial point clouds with and without using shapes from DSG-Net for data augmentation.
%Comparison of motion prediction on partial point clouds on whether using shapes from DSG-Net for data augmentation.
}
\label{tab:result_dsg}
\vspace{-6mm}
\end{table}



==> figures/tab_semiweakly_across_classes.tex <==
\begin{table*}[t]
\footnotesize
\addtolength{\tabcolsep}{-2pt}
\centering
%\begin{center}
\begin{tabular}{c|c|ccc|c|cc} \toprule 
% Category  & Method & Rotation Error   °↓      & Translation Error↓            & 3D IoU ↑                & Joint Error↓              & Angle Error°↓        & Distance Error↓              \\ \midrule 
\multirow{2}{*}{Category}           & \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Part-based Metrics}                                           & Joint States       & \multicolumn{2}{c}{Joint Parameters}      \\ 
                                    &                         & Rotation Error °↓         & Translation Error↓         & 3D IoU ↑                & Error↓             & Angle Error°↓      & Distance Error↓      \\ \midrule 
\multirow{3}{*}{mean}     & ANCSH   & 23.66  &	0.31 &	42.00 &	19.19 	& 3.25 &	0.04       \\
                          & ANCSH (Semi) & 24.76 & 0.32 & 41.00 & 22.21 & 3.39 & 0.06     \\
                         & ANCSH (Semi-weakly)       & \textbf{17.43} & \textbf{0.20} &	\textbf{44.85} &	\textbf{13.35} &	\textbf{2.62} &	\textbf{0.04} \\ \bottomrule 

\end{tabular}
% \caption{Result of semi-weakly supervised motion prediction.}
\caption{Averages of quantitative scores across object classes for Table 2 in our main paper.}
\label{tab:result_semiweakly_across_classes}
\end{table*}


==> figures/tab_statics.tex <==
% \begin{table}[h]
% % \scriptsize\addtolength{\tabcolsep}{-2pt}
% \footnotesize
% \addtolength{\tabcolsep}{-3pt}
% \centering
% %\begin{center}
% \begin{tabular}{c|ccc|ccc}\toprule
% Category & Part0 & Part1 & Part2 & Train & Test & Pseudo  \\ \midrule 

% refrigerator & Base & \makecell[c]{Left/Upper \\ door} & \makecell[c]{Right/Lower \\ door} & 22 & 3 & 67 \\
% dishwasher &  Base & Door & - & 34 & 5 & 91 \\
% table & Base & Drawer & - & 25 & 5 & 90  \\
% door\_set & Base & Door & - & 8 & 3 & 7  \\
% scissors & Handle & Handle & - & 37 & 6 & 62 \\ \bottomrule 
% \end{tabular}
% \caption{Part definitions of each category, together with the numbers of instances used for training and testing, and the pseudo-label instances selected by our method. }
% \label{tab:statics}
% \end{table}


\begin{table}[h]
% \scriptsize\addtolength{\tabcolsep}{-2pt}
\footnotesize
\addtolength{\tabcolsep}{-4pt}
\centering
%\begin{center}
\begin{tabular}{c|ccc|ccc}\toprule
Category & Part0 & Part1 & Part2 & Train & Test & Augmentation  \\ \midrule 

refrigerator & Base & \makecell[c]{Left/Upper \\ door} & \makecell[c]{Right/Lower \\ door} & 22 & 3 & 67 \\
dishwasher &  Base & Door & - & 34 & 5 & 91 \\
table & Base & Drawer & - & 25 & 5 & 90  \\
door\_set & Base & Door & - & 8 & 3 & 7  \\
scissors & Handle & Handle & - & 37 & 6 & 62 \\ \bottomrule 
\end{tabular}
\caption{Details about the number of samples per class. }
\label{tab:statics}
\end{table}


==> figures/tab_supervision_across_classes.tex <==
% \begin{table*}%[t!]
% \footnotesize\addtolength{\tabcolsep}{-2pt}
% \centering
% %\begin{center}
% \begin{tabular}{c|c|ccc|c|cc} \toprule 
% % Category  & Method & Rotation Error   °↓      & Translation Error↓            & 3D IoU ↑                & Joint Error↓              & Angle Error°↓        & Distance Error↓              \\ \midrule 
% \multirow{2}{*}{Category}           & \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Part-based Metrics}                                           & Joint States       & \multicolumn{2}{c}{Joint Parameters}      \\ 
%                                     &                         & Rotation Error °↓         & Translation Error↓         & 3D IoU ↑                & Error↓             & Angle Error°↓      & Distance Error↓      \\ \midrule 

                              
% \multirow{5}{*}{refrigerator} & Semi-weakly (100\%)           & \textbf{5.07   10.05 10.09} & \textbf{0.066 0.144 0.177} & \textbf{75.8 14.4 29.3} & \textbf{9.23 9.61} & \textbf{1.62 1.62} & \textbf{0.020 0.018} \\
%                               & Semi-weakly (80\%)            & \textbf{7.45 14.10 12.61}   & \textbf{0.096 0.171 0.188}          & \textbf{75.0 14.6 29.6}          & \textbf{12.62 10.98}        & 1.81 1.81          & \textbf{0.024 0.0192}         \\
%                               & Semi-weakly (50\%)            & \textbf{12.86 23.37 18.63}    & \textbf{0.147 0.464 0.430}         &     70.1 6.6 17.8       & \textbf{20.23 17.90}          &     2.99 2.88               & \textbf{0.033 0.031}            \\
%                               & Semi-weakly (30\%)            & 16.11 24.36 27.71           & 0.177 \textbf{0.516} \textbf{0.476}          & 71.7 \textbf{6.8 17.9}          & 18.59 22.11        & 1.83 1.82          & 0.039 \textbf{0.034}          \\ \cmidrule{2-8}
%                               & Supervised (100\%)            & 12.09 18.43 21.70         & 0.148 0.751 0.606          & 73.2 3.0 5.7            & 16.22 19.83        & 1.75 1.78          & 0.035 0.044          \\
%  \midrule

% \multirow{5}{*}{scissors}     & Semi-weakly (100\%)           & \textbf{12.00 13.52}        & \textbf{0.121 0.143}       & \textbf{37.2 37.8}      & \textbf{14.80}     & \textbf{2.10}      & \textbf{0.026}       \\
%                               & Semi-weakly   (80\%)          & 14.71 16.26                 & \textbf{0.142 0.165}       & \textbf{36.8 37.9}               & \textbf{18.38}              & \textbf{2.11}               & \textbf{0.027}                \\
%                               & Semi-weakly (50\%)            & \textbf{13.53} 18.17         & \textbf{0.162} 0.194                & 33.5 32.2               & 20.53              & 2.28               & 0.037                \\
%                               & Semi-weakly (30\%)            & \textbf{14.58} 18.29                 & 0.173 0.193                & 34.8 \textbf{35.5}               & \textbf{18.38}              & 2.38    & \textbf{0.033}         \\ \cmidrule{2-8}
%                               & Supervised (100\%)                      & 14.65 16.18               & 0.164 0.174                & 34.3 36.7               & 19.86              & 2.20                & 0.034                \\ \bottomrule 
% \end{tabular}
% %\end{center}
% \caption{Impact of different ratios of training data for supervision. We compare the performance \emph{ANCSH} trained using 100\% labeled data and \emph{ANCSH (Semi-weakly)} trained using  different ratios of labeled data, denoted as \emph{Supervised (100\%)} and \emph{Semi-weakly (*)}, respectively.
% Numbers for the semi-weakly supervised setting that outperform the 100\% supervised setting are bold.
% Note that our \emph{ANCSH (Semi-weakly)} is  comparable to \emph{Supervised (100\%)} even when only half of the labeled data is used.}
% \label{tab:result_supervision}
% \end{table*}


\begin{table*}%[t!]
\footnotesize\addtolength{\tabcolsep}{-2pt}
\centering
%\begin{center}
\begin{tabular}{c|c|ccc|c|cc} \toprule 
% Category  & Method & Rotation Error   °↓      & Translation Error↓            & 3D IoU ↑                & Joint Error↓              & Angle Error°↓        & Distance Error↓              \\ \midrule 
\multirow{2}{*}{Category}           & \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Part-based Metrics}                                           & Joint States       & \multicolumn{2}{c}{Joint Parameters}      \\ 
                                    &                         & Rotation Error °↓         & Translation Error↓         & 3D IoU ↑                & Error↓             & Angle Error°↓      & Distance Error↓      \\ \midrule 


\multirow{5}{*}{mean}     & Semi-weakly (100\%)           & \textbf{10.58} &	\textbf{0.13} &	\textbf{38.7} &	\textbf{12.11} &	\textbf{1.86} &	\textbf{0.023}   \\
                          & Semi-weakly   (80\%)          & \textbf{13.44} &	\textbf{0.15} &	\textbf{38.5} &	\textbf{15.09} &	\textbf{1.96} &	\textbf{0.025}  \\
                          & Semi-weakly (50\%)            & 17.07 &	\textbf{0.26} &	\textbf{32.2} &	19.80 &	2.61 &	\textbf{0.035} \\
                          & Semi-weakly (30\%)            &19.58 	& \textbf{0.29} &	\textbf{33.6} &	19.37 &	2.10 &	\textbf{0.035}   \\ \cmidrule{2-8}
                              & Supervised (100\%)        & 16.41 &	0.34 &	31.4 &	18.94 &	1.98 &	0.037  \\ \bottomrule 
\end{tabular}
%\end{center}
\caption{Averages of quantitative scores across object classes for Table 3 in our main paper.}
\label{tab:result_supervision_across_classes}
\end{table*}

